Model-based Testing of the Java Network API

Testing networked systems is challenging. The client or server side cannot be tested by itself. We present a solution using tool "Modbat" that generates test cases for Java's network library java.nio, where we test both blocking and non-blocking network functions. Our test model can dynamically simulate actions in multiple worker and client threads, thanks to a carefully orchestrated design that covers non-determinism while ensuring progress.

==> eptcsdata.tex <==
\providecommand{\firstpage}{46}
\providecommand{\publicationstatus}{J. Kofro\v{n}, J. Tumova (Eds.): Formal Engineering approaches\\
to Software Components and Architectures (FESCA'17)\\
EPTCS 245, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.245.4}{10.4204/EPTCS.245.4}}

